Variational Convergence of Discrete Minimal Surfaces

Building on and extending tools from variational analysis, we prove Kuratowski convergence of sets of simplicial area minimizers to minimizers of the smooth Douglas-Plateau problem under simplicial refinement. This convergence is with respect to a topology that is stronger than uniform convergence of both positions and surface normals.

==> Closedness.tex <==
\section{Closedness}

\begin{lemma}\label{lem:closednessofImmginstrongShape}
Let $\varSigma$ be a compact smooth manifold with boundary and let $\Curve \in \Imm(\partial\varSigma;\R^m)$ be a bi-Lipschitz homeomorphism onto its image.

Then $\strongShapeQuot(\Immg(\varSigma;\R^m))$ is a closed set in $\strongShape(\varSigma;\R^m)$.
\end{lemma}
\begin{proof}
It suffices to show that the invariant set
\begin{align*}
	\Immg(\varSigma;\R^m) \circ \Diff(\varSigma)
= (\strongShapeQuot)^{-1}(\strongShapeQuot(\Immg(\varSigma;\R^m)))
\end{align*}
 is closed in $(\strongImm(\varSigma;\R^m),\dstrongImm)$.

Let $f_n \in \strongImm(\varSigma;\R^m)$ 
and $\varphi_n \in \Diff(\varSigma)$ such that $f_n$ converges to some $f \in \strongImm(\varSigma;\R^m)$ in $\dstrongImm$
and such that $f_n \circ \varphi_n^{-1} \in \Immg(\varSigma;\R^m)$.
We have to find an $f \in \Imm(\varSigma;\R^m)$ and a $\varphi \in \Diff(\varSigma)$ with $f \circ \varphi^{-1} \in \Immg	(\varSigma;\R^m)$.

Of course, we cannot expect the $\varphi_n$ to converge in $\varSigma$.
However, we can show that $\psi_n \ceq \res(\varphi_n)$ is convergent:
One has $h_n \ceq \res(f_n) \converges{n \to \infty} h \ceq \res(f)$ in $\dstrongImm$ by \autoref{lem:strongImmhastrace}.
Observe $h_n = \Curve \circ \psi_n$, thus $h_n$ is actually a bi-Lipschitz homeomorphism onto $\Curve(\partial \varSigma)$. 
Since $\Curve(\partial \varSigma)$ is compact and thus closed, we also have $h(\partial \varSigma) \subset \Curve(\partial\varSigma)$ so that we may define $\psi \ceq \Curve^{-1} \circ h$.
This leads to
$\psi_n = \Curve^{-1} \circ h_n \converges{n\to \infty} \psi$ in $W^{1,\infty}_g$.
Moreover, one has
$\psi_n^{-1} = h_n^{-1} \circ \Curve$
and 
\begin{align*}
	T_{x}(\psi_n^{-1}) = 
	(T_{\psi_n^{-1}(x)}\psi_n)^\dagger = 	
	(\dd_{\psi_n^{-1}(x)} h_n)^\dagger\circ \dd_x \Curve
\end{align*}
for almost all $x \in \partial \varSigma$. This shows
$\nnorm{T(\psi_n^{-1})}_{L^\infty_g} \leq \nnorm{\dd  h_n^\dagger}_{L^\infty} \, \nnorm{\dd \Curve}_{L^\infty}$.
Since $(h_n)_{n\in\N}$ is bounded in $\dstrongImm$, the sequence $(\psi_n^{-1})_{n \in \N}$ is equicontinuous. 
This implies that there is a subsequence that converges to $\psi^{-1} \in C^0(\partial \varSigma;\partial\varSigma)$ in the compact-open topology and that $\psi^{-1}$ is Lipschitz continuous. Thus
$\psi \in \Diff(\partial \varSigma)$ is a bi-Lipschitz homeomorphism.
Now convergence $\psi_n \converges{n \to \infty} \psi$
in $W^{1,\infty}_{g_{\partial \varSigma}}(\partial \varSigma;\partial \varSigma)$ and $\psi \in \Diff(\partial \varSigma)$ together imply convergence
$\psi_n \converges{n \to \infty} \psi$ in $\Diff(\partial \varSigma)$.
As \autoref{lem:extendbnddiffeo} demonstrates, we can extend $\psi$ to a $\varphi \in \Diff(\varSigma)$ with $\res(\varphi) = \psi$. Finally,
$\res(f \circ \varphi^{-1}) = \res(f) \circ \res(\varphi^{-1}) = h \circ \psi^{-1} =\Curve$ completes the proof.
\qed
\end{proof}

\begin{lemma}\label{lem:extendbnddiffeo}
Let $\varphi_n \in \Diff(\varSigma)$ be a sequence of Lipschitz diffeomorphisms with $\res(\varphi_n) \converges{n\to \infty} \psi$ in $\Diff(\partial \varSigma)$.
Then there is $\varphi \in \Diff(\varSigma)$ with $\res(\varphi) = \psi$.
\end{lemma}
\begin{proof}
We choose a smooth Riemannian metric $g$ on $\partial \varSigma$.
Let $r>0$ be the geodesic radius of $(\partial \varSigma,g)$, i.e.,
for each $x \in \partial \varSigma$ the Riemannian exponential map
$\exp_x \colon K_x \to \partial \varSigma$
with $K_x \set{u \in T_x \partial \varSigma | \abs{u}_g \leq r}$ is a smooth diffeomorphism onto its image. 
%Since $K \ceq \bigcup_{x \in \partial \varSigma} K_x$ is compact, we may assume that $x\mapsto \dPosDefSec(\exp_x^\pull g,g\at_x)$ is uniformly bounded
Thus, for $n \in \N$ with $\sup_{x \in \varSigma} d_g(\psi(x),\psi_n(x)) <r$, there is a unique mapping $v_n \in W^{1,\infty}(\partial \varSigma;T\partial\varSigma)$ with $v_n(x) \in T_{\psi(x)}\varSigma$ with $\psi_n(x) = \exp( v_n(x))$. Now define
$H_n \colon \varSigma \times \intervalcc{0,1} \to \varSigma \times \intervalcc{0,1}$ by
$H_n(x,t) \ceq (\exp(t\, v_n(x)),t)$ and observe that $H_n$ is a Lipschitz diffeomorphism for sufficiently large $n$ and that $H_n(x,0) = (\psi(x),0)$ and $H_n(x,1) = (\psi_1(x),1)$ hold for all $x \in \partial \varSigma$.
Now, we fix such an $n \in \N$.

In order to transport $H_n$ to $\varSigma$, we choose a smooth collar $\varPhi \colon \partial \varSigma \times \intervalco{0,2} \to \varSigma$, i.e., a smooth embedding with $\varPhi(x,0)=x$ for all $x \in \partial \varSigma$.
We define the closed sets
$A \ceq \varPhi(\varSigma \times \intervalcc{0,1})$
and
$B \ceq \varSigma\setminus \varPhi(\partial \varSigma \times \intervalco{0,1})$.
We also shoose a smooth diffeomorphism $f \colon \varSigma \to B$ 
with $f\circ \varPhi(x,0) = \varPhi(x,1)$ for all $x \in \partial \varSigma$.
Note that $f|_{\partial \varSigma} \colon \partial \varSigma \to A\cap B$ is also a smooth diffeomorphism.
The mapping $\varphi_B \ceq f \circ \varphi_n \circ f^{-1} \colon B \to B$
and $\varphi_{A\cap B} \ceq (f|_{\partial \varSigma}) \circ \psi_n \circ (f|_{\partial \varSigma})^{-1} \colon A\cap B \to A \cap B$
are Lipschitz diffeomorhisms and one has $\varphi_B|_{A\cap B} = \varphi_{A\cap B}$.
Moreover, the mapping $\varphi_A = \varPhi|_{(\varSigma \times \intervalcc{0,1})} \circ H_n \circ (\varPhi|_{(\varSigma \times \intervalcc{0,1})})^{-1}$ 
is a Lipschitz diffeomorphism of $A$ and
satisfies $\varphi_A|_{\partial \varSigma} = \psi$ and $\varphi_A|_{A \cap B} = \varphi_{A\cap B}$.
Hence there is unique continuous map $\varphi \colon \varSigma \to \varSigma$
that makes the following diagramm commutative:
\begin{equation*}
\begin{tikzcd}[row sep=scriptsize, column sep=scriptsize]
	& A\cap B 
		\ar[dl, hook'] 
		\ar[rr, hook] 
		\ar[dr, hook] 		
		\ar[dd, near end, "\varphi_{A\cap B}"'] 
	& & 
	B 
		\ar[dl, hook'] 
		\ar[dd, "\varphi_B"] 
	\\ 
	A 
		\ar[rr, crossing over, hook] 
		\ar[dd, "\varphi_A"'] 
	& & 
	\varSigma 
	\\
	& A\cap B 
		\ar[dl, hook'] 
		\ar[rr, hook] 
		\ar[dr, hook] 		
	& & 
	B 
		\ar[dl, hook'] 
	\\ 
	A 
		\ar[rr, hook] 
	& & 
	\varSigma
		\ar[from=uu, crossing over, dashed, near start, "\varphi"]
\end{tikzcd}
\end{equation*}
The inverse $\varphi^{-1}$ exists and is also continuous. Both $\varphi$ and $\varphi^{-1}$ are piecewise of class $W^{1,\infty}$ and continuous. Thus,  we have $\varphi$, $\varphi^{-1} \in W^{1,\infty}(\varSigma;\varSigma)$, hence $\varphi \in \Diff(\varSigma)$. For $x \in \partial \varSigma \subset A$, we have $\varphi(x) = \varphi_A(x) = \varPhi( H_n(x,0))= \varPhi( \psi(x,0)) =\psi(x)$, hence $\res(\varphi) =\psi$ as desired.
\qed
\end{proof}
